Generalizing Few-Shot NAS with Gradient Matching

Efficient performance estimation of architectures drawn from large search spaces is essential to Neural Architecture Search. One-Shot methods tackle this challenge by training one supernet to approximate the performance of every architecture in the search space via weight-sharing, thereby drastically reducing the search cost. However, due to coupled optimization between child architectures caused by weight-sharing, One-Shot supernet's performance estimation could be inaccurate, leading to degraded search outcomes. To address this issue, Few-Shot NAS reduces the level of weight-sharing by splitting the One-Shot supernet into multiple separated sub-supernets via edge-wise (layer-wise) exhaustive partitioning. Since each partition of the supernet is not equally important, it necessitates the design of a more effective splitting criterion. In this work, we propose a gradient matching score (GM) that leverages gradient information at the shared weight for making informed splitting decisions. Intuitively, gradients from different child models can be used to identify whether they agree on how to update the shared modules, and subsequently to decide if they should share the same weight. Compared with exhaustive partitioning, the proposed criterion significantly reduces the branching factor per edge. This allows us to split more edges (layers) for a given budget, resulting in substantially improved performance as NAS search spaces usually include dozens of edges (layers). Extensive empirical evaluations of the proposed method on a wide range of search spaces (NASBench-201, DARTS, MobileNet Space), datasets (cifar10, cifar100, ImageNet) and search algorithms (DARTS, SNAS, RSPS, ProxylessNAS, OFA) demonstrate that it significantly outperforms its Few-Shot counterparts while surpassing previous comparable methods in terms of the accuracy of derived architectures.

==> cache.tex <==
\paragraph{Intro}
In recent years, there has been a surge of interest in Neural Architecture Search (NAS)~\citep{evolving, nas, enas, amoebanet, darts} for its ability to identify high-performing architectures in a series of machine learning tasks.
Pioneering works in this field require training and evaluating thousands of candidate architectures from scratch, which usually consume huge amounts of computational resources.
% Recently, one-shot NAS~\citep{enas, darts}, equipped with weight-sharing technique, has been proposed to drastically reduce the search cost down to that of training a single model.
% These method trains one single weight-sharing supernet (Shot) that encodes every architecture in the search space as a sub-path in the supernet, and subsequently use this supernet to efficiently estimate the performance of the underlying architectures.
To improve the search efficiency, one-shot NAS~\citep{enas, darts, oneshot} proposes to train one single weight-sharing supernet (Shot) that encodes every architecture in the search space as a sub-path in the supernet, and subsequently use this supernet to efficiently estimate the performance of the underlying architectures.
In the one-shot supernet, child models share weight with each other when their paths overlap.
One-Shot NAS methods manage to cut the search cost down to that of training a single model, while still achieve state-of-the-art performance.
% Due to the low search cost and competitive performance, one-shot NAS with weight sharing has been widely used.




However, due to coupled optimization between child models, the weight-sharing technique leads to inaccurate performance estimation, especially among top architectures~\citep{EvaluateSearch, pourchot2020share, zhang2020deeper, fewshotnas, xu2021analyzing}.
% Although one-shot NAS equipped with weight sharing has achieved success in many machine learning tasks, many works~\citep{EvaluateSearch, pourchot2020share, zhang2020deeper, fewshotnas, xu2021analyzing} criticized that the rank obtained using the supernet has a poor correlation with that obtained from the standalone training and this phenomenon is even more severe when applying weight sharing to large and complex search spaces.
% One-shot NAS suffers from the inaccurate performance rank ordering of candidate architectures due to the interference among candidate architectures during the training process. Poor correlation between the ranks obtained using the supernet and with the standalone training was observed by probing into several search spaces and the above phenomenon is even more severe for large and complex search spaces. 
% To alleviate the adverse effects caused by weight sharing, Few-Shot NAS~\citep{fewshotnas} proposes to split the single one-shot supernet into multiple sub-supernets via edge-wise exhaustive partitioning.
% Each supernet in few-shot NAS only contains architectures belonging to part of the search space. 
% The key problem in few-shot NAS can be formulated as a tree-splitting problem, i.e., how to split the supernet into several sub-supernets so that the interference among candidate architectures is minimised. 
% \citep{zhang2020deeper} sorts the candidate models lexicographcially and empirically slices the sorted candidate models into several groups while
% As shown in Figure~\ref{fig:comparison_gm_fewshot} (Right), each operation on the selected target edge is assigned to its own supernet.
% Few-Shot NAS exhaustively splits the supernet based on the number of operations in the randomly selected target edge. 
The exhaustive split method has the benefit of completely eliminating the weight-sharing w.r.t. the target edge, but needs to pay a cost of a high branching factor per split.
As a result, it can only afford to split a few edges due to the high computational overhead.
Given a fixed search budget, measured by the total number of leaf-node supernets, there exists a trade-off between width (branching factor) and depth (number of split) to minimize the adverse effect of weight sharing in different leaf-node supernets. 
Exhaustive split can be seen as a feasible solution to the interference minimization problem, which maximizes the tree width and significantly limits the depth.
However, it only considers the adverse effect of weight sharing at the selected edges and overlooks that at other edges, resulting in sub-optimal performance as NAS search space usually includes many edges.
Therefore, a more optimal solution to the above problem is to trade width for depth in the splitting tree, i.e. performing less splits per edge/layer, and split more edges/layers.
This necessitates a splitting criterion: how to decide which networks should or should not share weight with each other in the supernet?

A naive solution is to randomly split the operations with the assumption that weight sharing among all child models are equally harmful. 
However, empirically we found that this treatment barely matches the exhaustive splitting method used in~\citep{fewshotnas}, and in some cases worsen the performance.
The failure of the random split indicates that weight sharing among candidate networks are not equally harmful and motivates an explicit criterion to split child networks which are not suitable to share weight with others.
Intuitively, two candidate networks can share one copy of weight if the training dynamics of the shared modules is similar. 
This can be further verified from a multi-criteria optimization perspective~\citep{fliege2000steepest,brown2005directed}, i.e., by formulating the optimization of different child networks in one supernet as a multi-criteria optimization problem, only the similar update direction (training dynamic) can lead to the decrease of loss functions of all child networks, otherwise the performance of at least one child network will be deteriorated.
Inspired from the training dynamic of candidate networks, we propose to use gradient matching (GM) as the splitting criterion.
Concretely, consider two operations at a target edge to split, if these operations, when enabled separately, lead to different gradients on the shared edges, then we assign them to different sub-supernets.
By leveraging the gradient matching score as the splitting criterion, the supernet partition can be formulated as a graph min-cut problem as shown in the left part of Fig.~\ref{fig:comparison_gm_fewshot}, i.e., we first compute the gradient similarity from all pairs of operations on the target edge, which results in a densely connected graph, where the nodes are operations and edges are weighted by the gradient similarity measure;
then we perform the graph max-cut on this graph to split the operations (supernets) into several groups.
In the graph min-cut problem, each edge is assigned with a similarity score, which can serve as an edge importance measure to determine which edge to split next. 
Empirically, we found that our proposed GM method significantly outperforms the exhaustive splitting baseline in both performance rank ordering correlation and performance. 
We achieved 2.34\% test error on DARTS Space and a 19.7\% error on ImageNet task.
On NASBench-201, we also obtained state-of-the-art results on all three datasets.
